Internal Calibration Process Using Chirp Pulses with Application of the Adam Learning Algorithm

We propose a new internal calibration process using chirp pulses. Our method is utilized to mitigate thermal drift, which is unwanted changes and usually occurs in active elements such as a high power amplifier and low noise amplifier. The proposed method has advantages from two distinct aspects: calibration signal and algorithm. In respect to the calibration signal, our method does not contain an additional signal source because chirp pulses, which are normally used for remote sensing, are used as calibration signals. Moreover, our methods solve the ambiguity problem of analyzing a phase shift which occurs when sinusoidal signals are used as calibration signals. In regards to the algorithm, the Adam learning algorithm avoids learning in the wrong direction, unlike the conventional gradient descent. Using our method, mathematical forms of received signals are acquired successfully. Our method shows better effectivity compared to the conventional gradient descent algorithm. After compensation, the maximum differences of gain and phase become 0.06 dB and 2.42 degrees, respectively.

==> cite/README <==
This directory contains four .sty files that are mutually compatible,
but (mostly) independent:

cite.sty       Compressed, sorted lists of numerical citations: [8,11-16]
               with many options for controlling the formatting.

overcite.sty   like \usepackage[superscript]{cite}

drftcite.sty   Print the tags instead of the numbers for \cite and \bibitem.

chapterbib.sty Do multiple bibliographies--one for each \include file.

The user manuals for cite and chapterbib are LaTeX files cite.ltx
and chapterbib.ltx, and already typeset pdf versions.

They are all released under a very simple permissive license in
the MIT/BSD style:  They may be freely used, transmitted, reproduced, 
or modified provided that the copyright and permission notice is 
left intact.



Donald Arseneau                         asnd@triumf.ca

